Minimum Bisection is fixed parameter tractable

In the classic Minimum Bisection problem we are given as input a graph $G$ and an integer $k$. The task is to determine whether there is a partition of $V(G)$ into two parts $A$ and $B$ such that $||A|-|B|| \leq 1$ and there are at most $k$ edges with one endpoint in $A$ and the other in $B$. In this paper we give an algorithm for Minimum Bisection with running time $O(2^{O(k^{3})}n^3 \log^3 n)$. This is the first fixed parameter tractable algorithm for Minimum Bisection. At the core of our algorithm lies a new decomposition theorem that states that every graph $G$ can be decomposed by small separators into parts where each part is "highly connected" in the following sense: any cut of bounded size can separate only a limited number of vertices from each part of the decomposition. Our techniques generalize to the weighted setting, where we seek for a bisection of minimum weight among solutions that contain at most $k$ edges.

==> fig1.tex <==
\begin{tikzpicture}[scale=1.8]
  \tikzstyle{vertex}=[circle,fill=black,minimum size=0.20cm,inner sep=0pt]
  \tikzstyle{vertex2}=[circle,draw=black,fill=gray!50,minimum size=0.20cm,inner sep=0pt]
  \tikzstyle{terminal}=[rectangle,draw=black,fill=white,minimum size=0.2cm,inner sep=0pt]

\begin{scope}
\clip[rounded corners=60] (0,0) rectangle (4,3);
\fill[rounded corners=60,gray!50] (3,0) rectangle (7,3);
\fill[rounded corners=20,gray!50] (1.5,1.5) rectangle (5.5,2.5);
\end{scope}
\draw[rounded corners=60] (0,0) rectangle (4,3);
\draw[rounded corners=60] (3,0) rectangle (7,3);

\draw[rounded corners=20] (1.5,1.5) rectangle (5.5,2.5);

\draw[rounded corners] (2.5,2) -- (2.5,2.2) -- (3.7,2.2) -- (3.7,1.0) -- (3.3,1.0) -- (3.3,1.8) -- (2.5,1.8) -- (2.5,2);

\draw[rounded corners] (2,0.5) rectangle (2.8,1.3);
\draw (2.4,0.9) node {$D$};

\draw (0.5,2.5) node {$X$};
\draw (6.5,2.5) node {$Y$};
\draw (5,2) node {$S$};
\draw (3.4,2) node {$N(D)$};

%\begin{scope}
  %\clip (0,0) rectangle (10,10);
  %\fill[red] (3.5,3.5) circle (5);
%\end{scope}
%\draw (0,0) rectangle (10,10);
%\draw (3.5,3.5) circle (5) node {A};

	%\draw[rounded corners=20] (2,2) rectangle (6,4);
	%\draw[right] (6,3) node {$Q$};
	%\draw[rounded corners=10] (2.5,2.5) rectangle (4.5,3.5);

\end{tikzpicture}


==> fig2.tex <==
\begin{tikzpicture}[scale=1]
  \tikzstyle{vertex}=[circle,fill=black,minimum size=0.15cm,inner sep=0pt]
  \tikzstyle{vertex2}=[circle,draw=black,fill=gray!50,minimum size=0.20cm,inner sep=0pt]
  \tikzstyle{terminal}=[rectangle,draw=black,fill=white,minimum size=0.2cm,inner sep=0pt]


\draw[rounded corners=15] (0,0) rectangle (5,2);
\draw (2.5,1) ellipse (1 and 0.65);
\draw (4.5,1.5) node {$Q$};
\draw (2.5,1.3) node {$N(D_i)$};

\node[vertex] (a1) at (2,1){};
\node[vertex] (a2) at (2.5,1){};
\node[vertex] (a3) at (3,1){};

\foreach \i in {-1,0,1} {
	\draw[rounded corners] (1.75+\i * 3, -2) rectangle (1.75+\i*3+1.5,-1);
	\node[vertex] (x1) at (1.75+\i*3+1.5/4,-1.25){};
	\node[vertex] (x2) at (1.75+\i*3+2*1.5/4,-1.25){};
	\node[vertex] (x3) at (1.75+\i*3+3*1.5/4,-1.25){};
	\draw (x1) -- (a1);
	\draw (x2) -- (a1);
	\draw (x2) -- (a2);
	\draw (x2) -- (a3);
	\draw (x3) -- (a3);
}

\draw (-0.5,-1.7) node {$D_1$};
\draw (2.5,-1.7) node {$D_i$};
\draw (5.5,-1.7) node {$D_r$};

\draw (1,-1.5) node {$\ldots$};
\draw (4,-1.5) node {$\ldots$};


\end{tikzpicture}

